Saddlepoint Monte Carlo and its Application to Exact Ecological Inference

Assuming X is a random vector and A a non-invertible matrix, one sometimes need to perform inference while only having access to samples of Y = AX. The corresponding likelihood is typically intractable. One may still be able to perform exact Bayesian inference using a pseudo-marginal sampler, but this requires an unbiased estimator of the intractable likelihood. We propose saddlepoint Monte Carlo, a method for obtaining an unbiased estimate of the density of Y with very low variance, for any model belonging to an exponential family. Our method relies on importance sampling of the characteristic function, with insights brought by the standard saddlepoint approximation scheme with exponential tilting. We show that saddlepoint Monte Carlo makes it possible to perform exact inference on particularly challenging problems and datasets. We focus on the ecological inference problem, where one observes only aggregates at a fine level. We present in particular a study of the carryover of votes between the two rounds of various French elections, using the finest available data (number of votes for each candidate in about 60,000 polling stations over most of the French territory). We show that existing, popular approximate methods for ecological inference can lead to substantial bias, which saddlepoint Monte Carlo is immune from. We also present original results for the 2024 legislative elections on political centre-to-left and left-to-centre conversion rates when the far-right is present in the second round. Finally, we discuss other exciting applications for saddlepoint Monte Carlo, such as dealing with aggregate data in privacy or inverse problems.

==> applications_inverse.tex <==

\textbf{Methods for categorical ill-posed inverse problems}. Many works have been recently interested in ill-posed inverse problems, and among them ecological inference.

We find on the one hand works which rely on data augmentation and construct a
Markov chain on the possible values of $X$ given the observation $AX = b$ and
parameters $\theta$. A difficulty of the problem is that the admissible space
of $X | AX = b$ forms a discrete polytope with both equality and inequality
constraints, whose structure is difficult to manipulate.
\cite{airoldi2011polytope} directly tackle the geometrical difficulty and
proposes three conditional samplers of $X | AX = b$, with emphasis on the
uniform distribution. The problem is that, in the context of training models,
like with other data augmentation schemes, there is a very high correlation
between $X$ and $\theta$, meaning the solution will converge very slowly to the
solution. This also concerns other articles that propose ways of constructing
tables when conditioned on their margins (whose initial purpose was for
hypothesis testing), be it in a Metropolis-within-Gibbs approach
\citep{borkowf2004efficient} or directly a Gibbs approach
\citep{smith1996monte}. The same critique of poor mixing when training models
apply to modern sequential Monte Carlo methods \citep{chen2005sequential} which
also operate at a prohibitive cost. In addition, an issue of these works is
that they are highly dependent on the discrete nature of the data: our scheme
will work indiscriminately both for discrete and continuous $X$, as long as the
censoring filter $A$ is linear.

Recent developments in ill-posed inverse problems are found in machine learning
and computer vision. An issue is that, in this setting, it is not possible to
first train the model with some observed $X$ to then model the distribution of
$X | AX =b$, since only samples of $AX$ are available, which cuts our question
a good portion of the developments in plug-and-play methods in computer vision.
An adjacent and sometimes simpler goal consists of constructing estimators in
order to minimize the mean squared error in the parameter space, which can be
done without access to $X$ for Gaussian noise models using tricks such as
noise-to-noise \citep{lehtinen2018noise2noise}, noise-to-void
\citep{krull2019noise2void} and Tweedie's formula \citep{efron2011tweedie}
cannot easily apply. Methods relying on empirical Bayes least-squares
estimation have been proposed for other types of noises
\citep{raphan2011least}, but their reliance on the $\ell^2$ euclidean error (or
$\ell^1$ in some cases) makes them impractical when modeling data which do not
belong to euclidean spaces, such as with classification tasks.

Methods from the variational autoencoder literature could be used to perform
the inversion, but would also provide an approximation to the posterior
distribution because of how they rely on variational approximation schemes. On
the other hand, normalizing flows enable to perform exact posterior
distribution inference, but rely on an invertible mapping, which thus does not
apply simply to the setting where $A$ is non-invertible. Some recent interest
was found within surjective normalizing flows \citep{nielsen2020survae} and
could prove promising for categorical ill-posed inverse problems such as
ecological inference. Our scheme can be seen as an efficient method for
computing the likelihood resulting from an operation of the type $X \rightarrow
	AX$ with $A$ non-invertible, and we hypothesize it could be composed with other
tools from this literature. Other recent developments are found in optimal
transport for deconvolution problems and isotonic regression
\citep{carpentier2016learning, rigollet2019uncoupled}, which re-express these
in terms of an optimization problem that can be solved with the OT toolbox.
However, they suffer from the same issue that they rely on squared losses,
which is impractical when working on categorical data, and the cost may not be
learned, which means we may not define freely the generative model over $X$.
Unfortunately, OT methods that do enable learning the cost such as Sinkhorn-EM
\citep{mena2020sinkhorn} cannot be applied, for their two-marginals version, to
the problem of ecological inference, as $X$ is most often not a binary (but
rather Binomial or Poisson) variable. Finally, some recent interest was found
in describing the EI problem as a linear programming one
\citep{pavia2022improving}, but with a similar issue that it incurs the cost of
losing the possibility of freely formulating the underlying generating model
for $X$.

In conclusion, ill-posed (discrete) inverse problems have attracted
considerable attention from statisticians, machine learners and applied
mathematicians, but we have found no definite solution for our problem that is
simultaneously exact, that is very flexible and can work with various
functional forms, and that scales well to high dimension settings. We now
introduce saddlepoint Monte Carlo which is a good compromise between these
three aspects.


==> pres2024_full_france.tex <==
\begin{tabular}{lrrrrrrrrr}
\toprule
 & \multicolumn{3}{r}{Macron} & \multicolumn{3}{r}{Le Pen} & \multicolumn{3}{r}{Other} \\
 & .05 & .5 & .95 & .05 & .5 & .95 & .05 & .5 & .95 \\
\midrule
Macron & 0.92 & 0.92 & 0.92 & 0.05 & 0.05 & 0.05 & 0.03 & 0.03 & 0.03 \\
Le Pen & 0.00 & 0.00 & 0.00 & 0.97 & 0.97 & 0.97 & 0.03 & 0.03 & 0.03 \\
Melenchon & 0.47 & 0.47 & 0.47 & 0.00 & 0.00 & 0.00 & 0.53 & 0.53 & 0.54 \\
Other & 0.28 & 0.28 & 0.28 & 0.22 & 0.22 & 0.22 & 0.50 & 0.50 & 0.50 \\
\bottomrule
\end{tabular}

